LigoDV-web: Providing easy, secure and universal access to a large distributed scientific data store for the LIGO Scientific Collaboration

Gravitational-wave observatories around the world, including the Laser Interferometer Gravitational-wave Observatory (LIGO), record a large volume of gravitational-wave output data and auxiliary data about the instruments and their environments. These data are stored at the observatory sites and distributed to computing clusters for data analysis. LigoDV-web is a web-based data viewer that provides access to data recorded at the LIGO Hanford, LIGO Livingston and GEO600 observatories, and the 40m prototype interferometer at Caltech. The challenge addressed by this project is to provide meaningful visualizations of small data sets to anyone in the collaboration in a fast, secure and reliable manner with minimal software, hardware and training required of the end users. LigoDV-web is implemented as a Java Enterprise Application, with Shibboleth Single Sign On for authentication and authorization and a proprietary network protocol used for data access on the back end. Collaboration members with proper credentials can request data be displayed in any of several general formats from any Internet appliance that supports a modern browser with Javascript and minimal HTML5 support, including personal computers, smartphones, and tablets. To date 634 unique users have visited the LigoDV-web website in a total of 33,861 sessions and generated a total of 139,875 plots. This infrastructure has been helpful in many analyses within the collaboration including follow-up of the data surrounding the first gravitational-wave events observed by LIGO in 2015.

==> results.tex <==
a.	One or two examples of how ldvw has been used in Detchar to identify and track issues.
b.	Live Plot use during an ER.

Should we include here a step-by-step example of investigating a time series and spectrogram of one of the investigations in one of the recent detchar papers? Such as GW150914 or the S6 detchar paper? 
